Implementation of an Android Framework for USB storage access without root rights

This bachelor thesis describes the implementation of an Android framework to access mass storage devices over the USB interface of a smartphone. First the basics of USB (i.e. interfaces, endpoints and USB On the go) and accessing USB devices via the official Android API are discussed. Next the USB mass storage class is explained, which was de- signed by the USB-IF to access mobile mass storage like USB pen drives or external HDDs. For communication with mass storage devices, most important are the bulk-only transfer and the SCSI transparent command set. Furthermore file systems, for accessing directo- ries and files, are described. This thesis focuses on the FAT32 file system from Microsoft, because it is the most commonly used file system on such devices. After the theory part it is time to look at the implementation of the framework. In this section, the first concern is the purpose in general. Then the architecture of the framework and the actual implementation are presented. Important parts are discussed in detail. The thesis finishes with an overview of the test results on various Android devices, a short conclusion and an outlook to future developments. Moreover the current status of the developed framework is visualized.

==> components/abstract_german.tex <==
% German abstract for the CAMP report document
% Included by MAIN.TEX


\clearemptydoublepage






\vspace*{2cm}
\begin{center}
{\Large \bf Zusammenfassung}
\end{center}
\vspace{1cm}

Ultraschall ist ein weit verbreitetes bildgebendes Verfahren für die Diagnose und Verlaufskontrolle in vielen medizinischen Disziplinen. Die neueste Generation von Ultraschallsonden ist heutzutage in der Lage direkt 3D Bilder aufzunehmen, die meisten Ultraschallsysteme nehmen jedoch immer noch nur 2D Bilder auf. Für viele medizinische Anwendungen ist der klinische Nutzen von 2D Bilder nicht ausreichend. Es ist deshalb wünschenswert in der Lage zu sein 3D Bilder aufzunehmen. Eine bevorzugte Möglichkeit 3D Bilder, ohne eine 3D Ultraschallsonde, aufzunehmen ist eine Sequenz von 2D Ultraschallbildern aufzunehmen, während die Ultraschallsonde bewegt wird und dabei die Position und Orientierung der Ultraschallsonde aufzunehmen. Die aufgenommen Bilder und Positionsdaten können dann genutzt werden um ein 3D Bild zu erzeugen. Dafür muss aber die relative Lage des Ultraschallbildkoordinatensystems in Bezug zum Tracking Sensor Koordinatensystem bekannt sein, deshalb muss man eine Kalibrierung durchführen.

In der Literatur sind zahlreiche Methode beschrieben wie die Kalibrierung berechnet werden kann. Jedoch wurden die meisten dieser Methoden für die Forschung und prototypische Arbeit entwickelt und nicht für den Einsatz in einem industriellen Herstellungsprozess. Innerhalb dieser Arbeit haben wir eine Methode für die vollautomatische Kalibrierung für getrackte Ultraschallsonden entwickelt. Unsere Methode wurde mit dem Ziel die Kalibrierung von intravaskulären Ultraschallkathetern, mit integriertem magnetischen Trackingsensor, als Teil des Herstellungsprozess durchzuführen entwickelt. 




==> components/preface.tex <==
\clearemptydoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Preface}	


\vspace*{3cm}

\begin{flushleft}
{\Large \bf Preface}
\end{flushleft}

\vspace{1cm}




\newpage

==> components/text.tex <==
% Included by MAIN.TEX
% Put your content in here or include it by using \input (\include won't work)

\addtolength{\evensidemargin}{-12mm}

% ---------------------------------------------------------------------------
%
%Introduction and Background Theory
%
% ---------------------------------------------------------------------------
\part[Introduction and Background Theory]{Introduction and Background Theory}
\label{part:introAndBackgroundTheory}
\input{chapters/Introduction}
\input{chapters/BackgroundTheory} 

%
%% ---------------------------------------------------------------------------
%%
%% Fully Automated Calibration for Ultrasound
%%
%%% ---------------------------------------------------------------------------
\part[Fully Automated Calibration for Ultrasound]{Fully Automated Calibration for Ultrasound}
\label{part:fullyAutomatedCalibration}
\input{chapters/FullyAutomatedCalibrationOverview} 
\input{chapters/MethodsAndImplementation}
\input{chapters/SpheresPhantom} 
\input{chapters/ModulatedCirclesPhantom} 

%% ---------------------------------------------------------------------------
%%
%% Results and Conclusion
%%
%% ---------------------------------------------------------------------------
\part[Results and Conclusion]{Results and Conclusion}
\label{part:resultsAndConclusion}
\input{chapters/Experiments} 
\input{chapters/Simulations} 
\input{chapters/Conclusion} 


% ---------------------------------------------------------------------------
%
% Appendix
%
% ---------------------------------------------------------------------------

\part*{Appendix}
\addcontentsline{toc}{part}{Appendix}

\appendix %---------------------------------------

\input{chapters/validationDetailed}

